Rock, Rap, or Reggaeton?: Assessing Mexican Immigrants' Cultural Assimilation Using Facebook Data

The degree to which Mexican immigrants in the U.S. are assimilating culturally has been widely debated. To examine this question, we focus on musical taste, a key symbolic resource that signals the social positions of individuals. We adapt an assimilation metric from earlier work to analyze self-reported musical interests among immigrants in Facebook. We use the relative levels of interest in musical genres, where a similarity to the host population in musical preferences is treated as evidence of cultural assimilation. Contrary to skeptics of Mexican assimilation, we find significant cultural convergence even among first-generation immigrants, which problematizes their use as assimilative "benchmarks" in the literature. Further, 2nd generation Mexican Americans show high cultural convergence vis-\`a-vis both Anglos and African-Americans, with the exception of those who speak Spanish. Rather than conforming to a single assimilation path, our findings reveal how Mexican immigrants defy simple unilinear theoretical expectations and illuminate their uniquely heterogeneous character.

==> cross_demo_regression_table.tex <==
\begin{table}
\centering
\small
% old results with I=100 interests, no language
% \begin{tabular}{lccccc}
% & $\beta$ & S.E. & $t$ & $P>|t|$ & 95\% C.I. \\ 
% \midrule
% Intercept & 0.4603 & 0.033 & 14.085 & $<0.001$ & [0.396,0.524] \\
% \textbf{Gender} & ~ & ~ & ~ & ~ & ~ \\
% \hspace{10pt} Male & 0.0466 & 0.019 & 2.471 & 0.014 & [0.010,0.084] \\
% \textbf{Education} & ~ & ~ & ~ & ~ & ~ \\
% \hspace{10pt} High school graduate & -0.0739 & 0.027 & -2.768 & 0.006 & [-0.126,-0.022] \\
% \hspace{10pt} Less than high school graduate & 0.3409 & 0.027 & 12.779 & $<0.001$ & [0.289,0.393] \\
% \hspace{10pt} Two-year degree, Some college & 0.2041 & 0.027 & 7.649 & $<0.001$ & [0.152,0.256] \\
% \textbf{Age} & ~ & ~ & ~ & ~ & ~ \\
% \hspace{10pt} 19-28 & -0.8987 & 0.030 & -30.128 & $<0.001$ & [-0.957,-0.840] \\
% \hspace{10pt} 29-38 & -0.5761 & 0.030 & -19.313 & $<0.001$ & [-0.635,-0.518] \\
% \hspace{10pt} 39-48 & -0.3589 & 0.030 & -12.033 & $<0.001$ & [-0.417,-0.300] \\
% \hspace{10pt} 49-65 & -0.2108 & 0.030 & -7.065 & $<0.001$ & [-0.269,-0.152] \\
% \textbf{Region} & ~ & ~ & ~ & ~ & ~ \\
% \hspace{10pt} Northeast & -0.1227 & 0.027 & -4.598 & $<0.001$ & [-0.175,-0.070] \\
% \hspace{10pt} South & -0.1707 & 0.027 & -6.399 & $<0.001$ & [-0.223,-0.118] \\
% \hspace{10pt} West & -0.2508 & 0.027 & -9.400 & $<0.001$ & [-0.303,-0.198] \\
% \bottomrule
% \end{tabular}
\begin{tabular}{lrrrrc}
 & $\beta$ & S.E. & $t$ & $P>|t|$ & 95\% CI \\ 
\midrule
Intercept & 1.6960 & 0.054 & 31.268 & $<0.001$ & 1.590 1.802 \\
\textbf{Gender} & ~ & ~ & ~ & ~ & ~ \\
\hspace{10pt} Male & -0.0922 & 0.022 & -4.184 & $<0.001$ & [-0.135, -0.049] \\
\textbf{Region} & ~ & ~ & ~ & ~ & ~ \\
\hspace{10pt} Northeast & -0.1417 & 0.031 & -4.551 & $<0.001$ & [-0.203, -0.081] \\
\hspace{10pt} South & -0.2320 & 0.031 & -7.449 & $<0.001$ & [-0.293, -0.171] \\
\hspace{10pt} West & -0.2760 & 0.031 & -8.861 & $<0.001$ & [-0.337, -0.215] \\
\textbf{Age} & ~ & ~ & ~ & ~ & ~ \\
\hspace{10pt} 19-28 & -0.7611 & 0.035 & -21.856 & $<0.001$ & [-0.829, -0.693] \\
\hspace{10pt} 29-38 & -0.6281 & 0.035 & -18.037 & $<0.001$ & [-0.696, -0.560] \\
\hspace{10pt} 39-48 & -0.4348 & 0.035 & -12.485 & $<0.001$ & [-0.503, -0.366] \\
\hspace{10pt} 49-65 & -0.2318 & 0.035 & -6.656 & $<0.001$ & [-0.300, -0.163] \\
\textbf{Education} & ~ & ~ & ~ & ~ & ~ \\
\hspace{10pt} Bachelor's degree or more & -0.3532 & 0.031 & -11.340 & $<0.001$ & [-0.414, -0.292] \\
\hspace{10pt} High school graduate & -0.3972 & 0.031 & -12.752 & $<0.001$ & [-0.458, -0.336] \\
\hspace{10pt} Two-year degree,Some college & -0.0786 & 0.031 & -2.522 & 0.012 & [-0.140, -0.017] \\
\textbf{Language} & ~ & ~ & ~ & ~ & ~ \\
\hspace{10pt} Bilingual & -0.1231 & 0.027 & -4.564 & $<0.001$ & [-0.176, -0.070] \\
\hspace{10pt} Spanish & -0.3048 & 0.027 & -11.300 & $<0.001$ & [-0.358, -0.252] \\
\bottomrule
\end{tabular}
\caption{OLS regression results for predicting log assimilation score among Hispanic Mexican Ex-pats, across demographics. $N=2880, R^{2}=0.276, F=84.00 (p<$<0.001$)$. \todo{add interactions; do multiple step regression; reduce table to beta+SE+p-val}}
\label{tab:cross_demo_mx_expat_regression}
% src/analysis/compare_expat_subpopulation_assimilation.ipynb
\end{table}

==> cross_demo_regression_table_2.tex <==
\begin{table}[H]
\centering
\small
\begin{tabular}{l r r}
\toprule
~ & $\beta (SE)$ & p \\
\midrule
Intercept & 0.702 (0.024) & *** \\
\textbf{Gender} & ~ & ~ \\
\hspace{10pt}Female & 0.072 (0.013) & *** \\
\textbf{Education} & ~ & ~ \\
\hspace{10pt}High school graduate & -0.068 (0.018) & *** \\
\hspace{10pt}Less than high school graduate & 0.177 (0.018) & *** \\
Two-year degree,Some college & 0.151 (0.018) & *** \\
\textbf{Age} & ~ & ~ \\
\hspace{10pt}13-18 & 0.202 (0.021) & *** \\
\hspace{10pt}19-28 & -0.186 (0.021) & *** \\
\hspace{10pt}29-38 & -0.172 (0.021) & *** \\
\hspace{10pt}39-48 & -0.100 (0.021) & *** \\
\textbf{Language} & ~ & ~ \\
\hspace{10pt}Bilingual & 0.095 (0.016) & *** \\
\hspace{10pt}English & 0.175 (0.016) & *** \\
\textbf{Region} & ~ & ~ \\
\hspace{10pt}Midwest & 0.177 (0.018) & *** \\
\hspace{10pt}Northeast & 0.125 (0.018) & *** \\
\hspace{10pt}South & 0.041 (0.018) & * \\
\bottomrule
\end{tabular}
\caption{Regression results for cross-demographic assimilation comparison for first generation Hispanic Mexican expats. $N=3840, R^{2}=0.205, F=76.00 (p<0.001)$. *** $p<0.001$, ** $p<0.01$, * $p<0.05$.}
\label{tab:cross_demo_assimilation_gen_1}
\end{table}
\begin{table}[H]
\centering
\small
\begin{tabular}{l r r}
\toprule
~ & $\beta (SE)$ & p \\
\midrule
Intercept & 1.456 (0.026) & *** \\
\textbf{Gender} & ~ & ~ \\
\hspace{10pt}Female & 0.025 (0.014) & ~ \\
\textbf{Education} & ~ & ~ \\
\hspace{10pt}High school graduate & 0.023 (0.020) & * \\
\hspace{10pt}Less than high school graduate & 0.187 (0.020) & *** \\
\hspace{10pt}Two-year degree,Some college & 0.125 (0.020) & *** \\
\textbf{Age} & ~ & ~ \\
\hspace{10pt}13-18 & 0.091 (0.022) & *** \\
\hspace{10pt}19-28 & -0.255 (0.022) & *** \\
\hspace{10pt}29-38 & -0.125 (0.022) & *** \\
\hspace{10pt}39-48 & -0.048 (0.022) & * \\
\textbf{Language} & ~ & ~ \\
\hspace{10pt}Bilingual & -0.189 (0.017) & *** \\
\hspace{10pt}English & -0.215 (0.017) & *** \\
\textbf{Region} & ~ & ~ \\
\hspace{10pt}Midwest & 0.131 (0.020) & *** \\
\hspace{10pt}Northeast & 0.187 (0.020) & *** \\
\hspace{10pt}South & 0.034 (0.020) & * \\
\bottomrule
\end{tabular}
\caption{Regression results for cross-demographic assimilation comparison for second generation Hispanic Mexican expats. $N=3840, R^{2}=0.154, F=53.52 (p<0.001)$. *** $p<0.001$, ** $p<0.01$, * $p<0.05$.}
\label{tab:cross_demo_assimilation_gen_2}
\end{table}
% src/analysis/assimilation_regression.ipynb#Basic-regression

==> cross_demo_regression_table_african_american.tex <==
\begin{table}
\centering
\begin{tabular}{l r r}
\toprule
{} & $\beta (S.E.)$ & p \\
\midrule
Intercept & 0.357 (0.055) & *** \\
\textbf{Gender} & ~ & ~ \\
\hspace{8pt}Male & -0.188 (0.022) & *** \\
\textbf{Education} & ~ & ~ \\
\hspace{8pt}High school graduate & 0.051 (0.030) & ~ \\
\hspace{8pt}Less than high school graduate & -0.348 (0.031) & *** \\
\hspace{8pt}Two-year degree, Some college & -0.148 (0.031) & *** \\
\textbf{Age} & ~ & ~ \\
\hspace{8pt}19-28 & 1.182 (0.034) & *** \\
\hspace{8pt}29-38 & 1.013 (0.035) & *** \\
\hspace{8pt}39-48 & 0.815 (0.035) & *** \\
\hspace{8pt}49-65 & 0.599 (0.035) & *** \\
\textbf{Language} & ~ & ~ \\
\hspace{8pt}English & 0.420 (0.027) & *** \\
\hspace{8pt}Spanish & -1.124 (0.027) & *** \\
\textbf{Region} & ~ & ~ \\
\hspace{8pt}Northeast & -0.240 (0.034) & *** \\
\hspace{8pt}South & 0.462 (0.030) & *** \\
\hspace{8pt}West & 0.371 (0.030) & *** \\
\textbf{Generation} & ~ & ~ \\
\hspace{8pt}Generation 2+ & -1.095 (0.023) & *** \\
\bottomrule
\end{tabular}
\caption{Regression on log assimilation score with African Americans as the destination population. $N=28,203, R^{2}=0.215, F=552.9 (p<0.001)$. *** $p<0.001$, otherwise $p<0.05$.}
\label{tab:cross_demo_assim_african_american_regression}
% src/analysis/assimilation_regression.ipynb#Regression:-African-American
\end{table}

==> cross_demo_regression_table_anglo_interactions.tex <==
\begin{table*}
\small
\centering
\begin{tabular}{l r r r r r r}
\toprule
~ & \multicolumn{2}{l}{Model 1} & \multicolumn{2}{l}{Model 2} & \multicolumn{2}{l}{Model 3} \\
~ & \multicolumn{2}{l}{Age * Education} & \multicolumn{2}{l}{Age * Language} & \multicolumn{2}{l}{Age * Generation} \\ \midrule
~ & $\beta \:(S.E.)$ & $p$ & $\beta \:(S.E.)$ & $p$ & $\beta \:(S.E.)$ & $p$ \\
\midrule
Intercept & -1.460 (0.068) & *** & -1.243 (0.064) & *** & -1.316 (0.063) & *** \\
\textbf{Gender} & ~ & ~ & ~ & ~ & ~ & ~ \\
\hspace{8pt}Female & 0.276 (0.027) & *** & 0.265 (0.027) & *** & 0.274 (0.027) & *** \\
\textbf{Education} & ~ & ~ & ~ & ~ & ~ & ~ \\
\hspace{8pt}Bachelor's degree or more & -0.652 (0.086) & *** & 0.007 (0.036) & \textasciitilde & -0.009 (0.036) & \textasciitilde \\
\hspace{8pt}Less than high school graduate & -0.139 (0.083) & \textasciitilde & -0.404 (0.038) & *** & -0.387 (0.038) & *** \\
\hspace{8pt}Two-year degree, Some college & -0.895 (0.088) & *** & -0.200 (0.038) & *** & -0.204 (0.038) & *** \\
\textbf{Age} & ~ & ~ & ~ & ~ & ~ & ~ \\
\hspace{8pt}19-28 & 0.768 (0.081) & *** & 0.912 (0.068) & *** & 0.369 (0.070) & *** \\
\hspace{8pt}29-38 & 0.809 (0.082) & *** & 0.374 (0.071) & *** & 0.481 (0.070) & *** \\
\hspace{8pt}39-48 & 0.620 (0.081) & *** & 0.163 (0.072) & \textasciitilde & 0.540 (0.070) & *** \\
\hspace{8pt}49-65 & 0.442 (0.081) & *** & 0.112 (0.073) & \textasciitilde & 0.512 (0.070) & *** \\
\textbf{Language} & ~ & ~ & ~ & ~ & ~ & ~ \\
\hspace{8pt}Bilingual & 1.196 (0.033) & *** & 0.338 (0.075) & *** & 1.186 (0.033) & *** \\
\hspace{8pt}English & 1.663 (0.032) & *** & 1.091 (0.074) & *** & 1.654 (0.032) & *** \\
\textbf{Region} & ~ & ~ & ~ & ~ & ~ & ~ \\
\hspace{8pt}Midwest & -0.524 (0.036) & *** & -0.510 (0.036) & *** & -0.514 (0.036) & *** \\
\hspace{8pt}Northeast & -0.828 (0.041) & *** & -0.827 (0.041) & *** & -0.836 (0.041) & *** \\
\hspace{8pt}West & -0.150 (0.035) & *** & -0.142 (0.035) & *** & -0.144 (0.035) & *** \\
\textbf{Generation} & ~ & ~ & ~ & ~ & ~ & ~ \\
\hspace{8pt}Generation 2+ & -1.130 (0.028) & *** & -1.121 (0.028) & *** & -1.735 (0.064) & *** \\
\textbf{Model 1} & ~ & ~ & ~ & ~ & ~ & ~ \\
\hspace{8pt}19-28*Bachelor's degree or more & 0.851 (0.118) & *** & ~ & ~ & ~ & ~ \\
\hspace{8pt}29-38*Bachelor's degree or more & 0.687 (0.118) & *** & ~ & ~ & ~ & ~ \\
\hspace{8pt}39-48*Bachelor's degree or more & 0.674 (0.118) & *** & ~ & ~ & ~ & ~ \\
\hspace{8pt}49-65*Bachelor's degree or more & 0.945 (0.118) & *** & ~ & ~ & ~ & ~ \\
\hspace{8pt}19-28*Less than high school graduate & 0.002 (0.116) & \textasciitilde & ~ & ~ & ~ & ~ \\
\hspace{8pt}29-38*Less than high school graduate & -0.540 (0.118) & *** & ~ & ~ & ~ & ~ \\
\hspace{8pt}39-48*Less than high school graduate & -0.407 (0.119) & ** & ~ & ~ & ~ & ~ \\
\hspace{8pt}49-65*Less than high school graduate & -0.381 (0.121) & \textasciitilde & ~ & ~ & ~ & ~ \\
\hspace{8pt}19-28*Two-year degree,Some college & 0.955 (0.119) & *** & ~ & ~ & ~ & ~ \\
\hspace{8pt}29-38*Two-year degree,Some college & 0.790 (0.121) & *** & ~ & ~ & ~ & ~ \\
\hspace{8pt}39-48*Two-year degree,Some college & 0.961 (0.121) & *** & ~ & ~ & ~ & ~ \\
\hspace{8pt}49-65*Two-year degree,Some college & 0.715 (0.122) & *** & ~ & ~ & ~ & ~ \\
\textbf{Model 2} & ~ & ~ & ~ & ~ & ~ & ~ \\
\hspace{8pt}19-28*Bilingual & ~ & ~ & 0.663 (0.102) & *** & ~ & ~ \\
\hspace{8pt}29-38*Bilingual & ~ & ~ & 1.200 (0.104) & *** & ~ & ~ \\
\hspace{8pt}39-48*Bilingual & ~ & ~ & 1.304 (0.105) & *** & ~ & ~ \\
\hspace{8pt}49-65*Bilingual & ~ & ~ & 1.032 (0.106) & *** & ~ & ~ \\
\hspace{8pt}19-28*English & ~ & ~ & 0.139 (0.101) & \textasciitilde & ~ & ~ \\
\hspace{8pt}29-38*English & ~ & ~ & 0.780 (0.103) & *** & ~ & ~ \\
\hspace{8pt}39-48*English & ~ & ~ & 0.960 (0.104) & *** & ~ & ~ \\
\hspace{8pt}49-65*English & ~ & ~ & 0.907 (0.105) & *** & ~ & ~ \\
\textbf{Model 3} & ~ & ~ & ~ & ~ & ~ & ~ \\
\hspace{8pt}19-28*Generation 2+ & ~ & ~ & ~ & ~ & 1.257 (0.088) & *** \\
\hspace{8pt}29-38*Generation 2+ & ~ & ~ & ~ & ~ & 0.843 (0.088) & *** \\
\hspace{8pt}39-48*Generation 2+ & ~ & ~ & ~ & ~ & 0.570 (0.089) & *** \\
\hspace{8pt}49-65*Generation 2+ & ~ & ~ & ~ & ~ & 0.372 (0.089) & *** \\
\bottomrule
\end{tabular}
\caption{Regression on log assimilation score with Anglo Americans as the destination population, using three models to handle interaction between independent variables. *** indicates $p<0.001$, ** $p<0.01$, * $p<0.05$, otherwise $p>0.05$ (after applying Bonferroni correction for multiple hypotheses).}
\label{tab:cross_demo_assim_anglo_regression_interactions}
% src/analysis/assimilation_regression.ipynb#Control-for-interaction-effects
\end{table*}

==> ethnicity_assim_scores_table.tex <==
\begin{table}
\small
\centering
\begin{tabular}{l l r}
Ethnic group & Interest name & $AR$ \\
\rowcolor{Gray}
\textbf{White} & ~ & ~ \\
~ & Australian folk music & 0.280 \\
~ & Old-time music & 0.276 \\
~ & Canadian rock & 0.203 \\
~ & Folk music of Ireland & 0.194 \\
~ & Marching band & 0.002 \\
\rowcolor{Gray}
\textbf{African American} & ~ & ~ \\
~ & Atlanta hip hop & 0.200 \\
~ & R\&B/Soul & 0.188 \\
~ & Soul jazz & 0.106 \\
~ & Urban contemporary gospel & 0.093 \\
~ & Marching band & 0.003 \\
% \rowcolor{Gray}
% \textbf{Hispanic} & ~ & ~ \\
% ~ & Outlaw country & 0.553 \\
% ~ & Texas country music & 0.530 \\
% ~ & Red Dirt (music) & 0.520 \\
% ~ & Music of Texas & 0.503 \\
% ~ & Horror punk & 0.005 \\ \hline
\end{tabular}
% src/analysis/compare_non_expat_subpopulation_assimilation.ipynb#Low/high-scoring-ethnic-assimilation-scores
\caption{The five lowest-scoring musical interests for first-generation Hispanic Mexican immigrants, compared to each ethnic group. \todo{ALL THE GENERATIONS}}
\label{tab:ethnic_assim_scores_examples}
\end{table}

==> generation_assim_scores_table.tex <==
\begin{table}
\centering
\small

% 4 columns
% \begin{tabular}{l p{4cm} p{4cm} p{4cm} p{4cm}}
% ~ & Hispanic\_MX\_1 & Hispanic\_MX\_2\_communities & Hispanic\_MX\_2\_Spanish & Hispanic\_MX\_2\_interest \\
% \midrule
% 1 & Criolla & Criolla & Music of Mexico & Music of Mexico \\
% 2 & Music of Mexico & Music of Mexico & Hot R\&B/Hip-Hop Songs & Urban contemporary gospel \\
% 3 & Trova & Urban contemporary gospel & West Coast hip hop & Mento \\
% 4 & Timba & Timba & Southern hip hop & Chicago hip hop \\
% 5 & Mento & Mento & Bouyon music & Slow jam \\
% 6 & UK funky & Slow jam & Spoken word & Roots reggae \\
% 7 & Urban contemporary gospel & Trova & Space age pop & Crunk \\
% 8 & Guajira (music) & Crunk & Electro house & Trova \\
% 9 & Latin dance & Roots reggae & Roots reggae & Bouyon music \\
% 10 & Zouk (club) & Guajira (music) & Crunk & Southern hip hop \\
% \bottomrule
% \end{tabular}

% 2 columns
\begin{tabular}{lll}
\rowcolor{Gray}
Rank & \textbf{Hispanic\_MX\_1} & \textbf{Hispanic\_MX\_2\_communities} \\ 
1 & Criolla (175.40) & Criolla (35.81) \\
2 & Music of Mexico (46.17) & Music of Mexico (24.46) \\
3 & Trova (40.20) & Urban contemporary gospel (11.55) \\
4 & Timba (29.51) & Timba (9.94) \\
5 & Mento (17.29) & Mento (8.78) \\
6 & UK funky (9.28) & Slow jam (8.63) \\
7 & Urban contemporary gospel (8.71) & Trova (7.53) \\
8 & Guajira (music) (7.66) & Crunk (5.71) \\
9 & Latin dance (6.45) & Roots reggae (5.32) \\
10 & Zouk (club) (4.53) & Guajira (music) (5.29) \\ 
\rowcolor{Gray}
~ & \textbf{Hispanic\_MX\_2\_Spanish} & \textbf{Hispanic\_MX\_2\_interest} \\
1 & Music of Mexico (77.05) & Music of Mexico (18.05) \\
2 & Hot R\&B/Hip-Hop Songs (3.85) & Urban contemporary gospel (11.77) \\
3 & West Coast hip hop (2.20) & Mento (8.95) \\
4 & Southern hip hop (2.17) & Chicago hip hop (7.32) \\
5 & Bouyon music (2.12) & Slow jam (6.86) \\
6 & Spoken word (1.43) & Roots reggae (5.19) \\
7 & Space age pop (1.39) & Crunk (5.04) \\
8 & Electro house (1.33) & Trova (4.98) \\
9 & Roots reggae (1.25) & Bouyon music (4.15) \\
10 & Crunk (1.19) & Southern hip hop (3.97) \\ \bottomrule
\end{tabular}
\caption{Top-10 interests by assimilation score for each generation category.}
\label{tab:top_k_assim_scores_generation}
% src/analysis/compare_non_expat_subpopulation_assimilation.ipynb#Top-k assimilation scores per generation
\end{table}
